Continual Learning of Numerous Tasks from Long-tail Distributions

Continual learning, an important aspect of artificial intelligence and machine learning research, focuses on developing models that learn and adapt to new tasks while retaining previously acquired knowledge. Existing continual learning algorithms usually involve a small number of tasks with uniform sizes and may not accurately represent real-world learning scenarios. In this paper, we investigate the performance of continual learning algorithms with a large number of tasks drawn from a task distribution that is long-tail in terms of task sizes. We design one synthetic dataset and two real-world continual learning datasets to evaluate the performance of existing algorithms in such a setting. Moreover, we study an overlooked factor in continual learning, the optimizer states, e.g. first and second moments in the Adam optimizer, and investigate how it can be used to improve continual learning performance. We propose a method that reuses the optimizer states in Adam by maintaining a weighted average of the second moments from previous tasks. We demonstrate that our method, compatible with most existing continual learning algorithms, effectively reduces forgetting with only a small amount of additional computational or memory costs, and provides further improvements on existing continual learning algorithms, particularly in a long-tail task sequence.

==> experiments_v1.tex <==
\section{Experiments}
% \begin{table}[]
%     \centering
%     \caption[Synthetic task results.]{Results of synthetic task where $d=128$, 5 tasks, and $\mathbf{w}$ for all tasks are the same. Reported numbers are the mean of 1000 runs.}
%     \begin{tabular}{ccccc}
%     \hline
%     Method           & RA↓    & BWT↑  & FGT↓  & LA↓    \\ \hline
%     Moment-continual & 1.46  & -1.41 & 1.41 & 0.051 \\
%     Moment-reset     & 1.91  & -1.85 & 1.86 & 0.051 \\
%     MTL              & 0.047 & -    & -    & -     \\ \hline
%     \end{tabular}
%     \label{tab:synthetic_same_w}
% \end{table}

\begin{table}[htbp]
    \centering
    \caption[Synthetic task results.]{Results of synthetic task where $d=128$, 5 tasks, and $\mathbf{w}$ for all tasks are the same. }%Reported numbers are the mean of 1000 runs.}
\begin{tabular}{cllllllll}
\hline
\multicolumn{1}{l}{} & \multicolumn{2}{c}{RA↓}                             & \multicolumn{2}{c}{BWT↓}                            & \multicolumn{2}{c}{FGT↓}                            & \multicolumn{2}{c}{LA↓}                               \\
Method               & \multicolumn{1}{c}{MC}   & \multicolumn{1}{c}{MR}   & \multicolumn{1}{c}{MC}   & \multicolumn{1}{c}{MR}   & \multicolumn{1}{c}{MC}   & \multicolumn{1}{c}{MR}   & \multicolumn{1}{c}{MC}    & \multicolumn{1}{c}{MR}    \\ \hline
Adam                 & \multicolumn{1}{c}{1.46} & \multicolumn{1}{c}{1.91} & \multicolumn{1}{c}{1.41} & \multicolumn{1}{c}{1.85} & \multicolumn{1}{c}{1.41} & \multicolumn{1}{c}{1.86} & \multicolumn{1}{c}{0.051} & \multicolumn{1}{c}{0.051} \\
Reservoir            &                          &                          &                          &                          &                          &                          &                           &                           \\
DER++                &                          &                          &                          &                          &                          &                          &                           &                           \\
AGEM                 &                          &                          &                          &                          &                          &                          &                           &                           \\
EWC++                  &                          &                          &                          &                          &                          &                          &                           &                           \\
MTL                  & \multicolumn{2}{c}{0.047}                           & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{-}     \\ \hline
\end{tabular}
\end{table}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{images/diff_by_k.png}
    \caption[Effect of task diversity.]{From left to right: 1) Difference between MC and MR vs. diversity of task; 2)Average loss over all tasks at the end vs. tail thickness of task sizes distribution; 3) }
    \label{fig:synthetic_plots}
\end{figure}

%
\begin{table}[htbp]
    \centering
    \caption[Moment-continual Optimizer results, long-tail ordering.]{Comparison between Moment-continual (MC) and Moment-reset (MR) Optimizers or WSD-CL. Task ordered by sampling by task sizes without replacement. }%Numbers reported are \emph{example}-wise metrics.}
    \label{tab:mr_vs_mc_freq}
    \resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
    \hline
    \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{2}{c}{RA↑}   & \multicolumn{2}{c}{BWT↑}   & \multicolumn{2}{c}{FGT↓} & \multicolumn{2}{c}{LA↑}   \\
    Buffer                   & Method               & MC          & MR          & MC          & MR           & MC         & MR          & MC          & MR          \\ \hline
    \multirow{2}{*}{0}       & Fine-tuning          & 77.72 & 65.29 & -2.36 & -14.35 & 7.11 & 21.79 & 80.09 & 79.65 \\
                             & EWC++                & 76.68 & 73.48 & -2.59 & -5.65  & 7.82 & 10.30 & 79.27 & 79.14 \\ \hline
    \multirow{3}{*}{200}     & Reservoir            & 77.92 & 66.34 & -1.85 & -12.87 & 6.80 & 20.46 & 79.78 & 79.21 \\
                             & DER++                & 74.29 & 73.85 & -4.15 & -5.86  & 9.67 & 10.39 & 78.44 & 79.71 \\
                             & AGEM                 & 76.53 & 66.20 & -3.55 & -13.41 & 8.37 & 20.57 & 80.08 & 79.61 \\ \hline
    \multirow{3}{*}{2000}    & Reservoir            & 78.01 & 72.10 & -1.73 & -6.73  & 6.37 & 13.49 & 79.74 & 78.83 \\
                             & DER++                & 78.12 & 77.17 & -1.26 & -2.40  & 6.10 & 6.42  & 79.38 & 79.56 \\
                             & AGEM                 & 77.87 & 67.06 & -2.09 & -12.13 & 6.88 & 18.75 & 79.96 & 79.19 \\ \hline
    \multirow{3}{*}{20000}   & Reservoir            & 78.92 & 75.65 & -0.53 & -3.60  & 5.45 & 8.31  & 79.45 & 79.25 \\
                             & DER++                & 79.57 & 78.13 & -0.10 & -1.01  & 4.48 & 4.46  & 79.67 & 79.14 \\
                             & AGEM                 & 77.83 & 71.65 & -2.06 & -7.62  & 6.95 & 13.88 & 79.89 & 79.28 \\ \hline
    \multirow{4}{*}{2000000} & Reservoir            & 81.00 & 78.36 & 0.89  & -1.35  & 4.11 & 5.92  & 80.11 & 79.71 \\
                             & DER++                & 79.08 & 78.58 & 0.76  & -0.43  & 4.33 & 4.35  & 78.32 & 79.01 \\
                             & AGEM                 & 78.61 & 73.56 & -1.48 & -6.23  & 6.35 & 12.22 & 80.09 & 79.79 \\
                             & MbPA++               & 80.05 & 64.89 & -0.01 & -14.52 & 2.28 & 17.44 & 80.06 & 79.40 \\ \hline
    \end{tabular}
    }
\end{table}

\begin{table}[htbp]
    \centering
    \caption[Moment-continual Optimizer results, random ordering.]{Comparison between Moment-continual (MC) and Moment-reset (MR) Optimizers on WSD-CL. Task ordered randomly. }%Numbers reported are \emph{example}-wise metrics.}
    \label{tab:mr_vs_mc_freq}
    \resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
    \hline
    \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{2}{c}{RA↑}   & \multicolumn{2}{c}{BWT↑}  & \multicolumn{2}{c}{FGT↓} & \multicolumn{2}{c}{LA↑}   \\
    Buffer                   & Method               & MC          & MR          & MC          & MR          & MC         & MR          & MC          & MR          \\ \hline
    \multirow{2}{*}{0}       & Fine-tuning          & 78.69 & 76.61 & -0.26 & -1.94 & 8.01 & 9.58  & 78.96 & 78.55 \\
                             & EWC++                & 75.96 & 73.77 & -0.25 & -0.18 & 7.72 & 7.04  & 76.21 & 73.95 \\ \hline
    \multirow{3}{*}{200}     & Reservoir            & 78.50 & 75.13 & -0.22 & -3.33 & 8.16 & 10.96 & 78.72 & 78.46 \\
                             & DER++                & 78.16 & 76.53 & -0.66 & -1.88 & 8.29 & 9.48  & 78.82 & 78.41 \\
                             & AGEM                 & 78.33 & 76.25 & -0.31 & -2.24 & 8.07 & 10.03 & 78.64 & 78.50 \\ \hline
    \multirow{3}{*}{2000}    & Reservoir            & 78.35 & 75.48 & -0.24 & -2.58 & 7.66 & 9.73  & 78.60 & 78.07 \\
                             & DER++                & 78.76 & 77.37 & 0.33  & -0.96 & 6.64 & 7.53  & 78.43 & 78.33 \\
                             & AGEM                 & 77.51 & 75.82 & 0.11  & -2.67 & 8.42 & 10.28 & 77.40 & 78.49 \\ \hline
    \multirow{3}{*}{20000}   & Reservoir            & 79.43 & 77.46 & 0.43  & -1.47 & 6.36 & 7.91  & 78.99 & 78.93 \\
                             & DER++                & 79.62 & 78.76 & 1.15  & 0.25  & 5.06 & 5.43  & 78.47 & 78.51 \\
                             & AGEM                 & 78.86 & 77.45 & -0.12 & -1.49 & 7.48 & 8.70  & 78.99 & 78.95 \\ \hline
    \multirow{4}{*}{2000000} & Reservoir            & 81.73 & 80.93 & 2.31  & 1.37  & 4.84 & 5.11  & 79.42 & 79.56 \\
                             & DER++                & 80.95 & 80.35 & 2.20  & 1.84  & 4.11 & 4.11  & 78.76 & 78.52 \\
                             & AGEM                 & 79.24 & 77.94 & 0.23  & -1.09 & 7.42 & 8.26  & 79.01 & 79.03 \\
                             & MbPA++               & 79.50 & 77.33 & 0.36  & -1.73 & 3.30 & 5.29  & 79.14 & 79.05 \\ \hline
    \end{tabular}
    }
\end{table}
%

\begin{table}[htbp]
    \centering
    \caption{Results on image classification continual learning. Average accuracy over all tasks after learning the last task. Numbers reported are average of 10 runs. TODO: results in bracket is using algorithm 1}
    \label{tab:my_label}
\begin{tabular}{cccclcl}
\hline
\multicolumn{1}{l}{} & \multicolumn{2}{c}{MNIST}                   & \multicolumn{2}{c}{CIFAR10}                      & \multicolumn{2}{c}{CIFAR100}                     \\
Method               & MC                   & MR                   & MC                   & \multicolumn{1}{c}{MR}    & MC                   & \multicolumn{1}{c}{MR}    \\ \hline
Finetune                  & 19.24(19.09)                & 18.77                &  19.61(19.58)         & 19.58         & 10.22 & 10.20                  \\
EWC++                  & 19.65(19.07)                & 18.96                & 18.99(19.34)                & 17.68                    & 8.91 & 8.84                      \\
Reservoir            &                      &                      &                      & \multicolumn{1}{c}{}      &                      & \multicolumn{1}{c}{}      \\
DER++                & 86.48(86.17)                & 85.85                & 62.04                & \multicolumn{1}{c}{61.10} & 35.88                & \multicolumn{1}{c}{34.96} \\
AGEM                  & 74.05(73.24)                & 71.46                & 27.70                &     21.06                 & \multicolumn{1}{l}{} &                           \\
MTL                  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                           & \multicolumn{1}{l}{} &                           \\ \hline
\end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Continual learning on 5 NLP task: SQuAD, WikiSQL, SST, QA-SRL, WOZ. Formatted as QA tasks, using GPT2 as backbone. }
\begin{tabular}{cllclclcl}
\hline
\multicolumn{1}{l}{} & \multicolumn{2}{c}{RA↑}                         & \multicolumn{2}{c}{BWT↑}                      & \multicolumn{2}{c}{FGT↓}                      & \multicolumn{2}{c}{LA↑}                       \\
Method               & \multicolumn{1}{c}{MC} & \multicolumn{1}{c}{MR} & MC                   & \multicolumn{1}{c}{MR} & MC                   & \multicolumn{1}{c}{MR} & MC                   & \multicolumn{1}{c}{MR} \\ \hline
Finetune             &                        &                        & \multicolumn{1}{l}{} &                        & \multicolumn{1}{l}{} &                        & \multicolumn{1}{l}{} &                        \\
Reservoir            &                        &                        & \multicolumn{1}{l}{} &                        & \multicolumn{1}{l}{} &                        & \multicolumn{1}{l}{} &                        \\
MTL                  & \multicolumn{2}{l}{}                            & -                    & \multicolumn{1}{c}{-}  & -                    & \multicolumn{1}{c}{-}  & -                    & \multicolumn{1}{c}{-}  \\ \hline
\end{tabular}
\end{table}
